Sampling NNLO QCD phase space with normalizing flows

We showcase the application of neural importance sampling for the evaluation of NNLO QCD scattering cross sections. We consider Normalizing Flows in the form of discrete Coupling Layers and time continuous flows for the integration of the various cross-section contributions when using the sector-improved residue subtraction scheme. We thereby consider the stratification of the integrands into their positive and negative contributions, and separately optimize the phase-space sampler. We exemplify the novel methods for the case of gluonic top-quark pair production at the LHC at NNLO QCD accuracy. We find significant gains with respect to the current default methods used in STRIPPER in terms of reduced cross-section variances and increased unweighting efficiencies. In turn, the computational costs for evaluations of the integrand needed to achieve a certain statistical uncertainty for the cross section can be reduced by a factor 8.

==> table-performance-NLO.tex <==
Contribution $\sigma^i$ & & & $\sigma^{\mathrm{B}} \cdot 10^{-2}$& & $\sigma^{\mathrm{RF}} \cdot 10^{-2}$& & $\sigma^{\mathrm{RU}} \cdot 10^{-2}$& & $\sigma^{\mathrm{VF}} \cdot 10^{-1}$& \\
$\delta_{\mathrm{opt}}$ [pb] & & &  0.0001& &  0.008& &  0.01& &  0.006& \\
cost $C_i$ [a.u.] & & & 1& & 6& & 2& & 1& \\
% \hat{\sigma}
$\hat{\sigma} \pm \delta \hat{\sigma}\,\text{[pb]}$& & \Vegas &  5.328 \pm 0.002& &  6.97 \pm 0.01& &  -5.38 \pm 0.02& &  -4.487 \pm 0.006& \\
& & \textsc{Ode} &  5.3279 \pm 0.0005& &  6.980 \pm 0.009& &  -5.39 \pm 0.01& &  -4.483 \pm 0.006& \\
& & \textsc{Cl} &  5.3280 \pm 0.0003& &  6.972 \pm 0.009& &  -5.39 \pm 0.01& &  -4.492 \pm 0.006& \\
\addlinespace
% \hat{\sigma}^+
$\hat{\sigma}^+ \pm \delta \hat{\sigma}^+ \,\text{[pb]}$& & \Vegas &  5.328 \pm 0.002& &  8.96 \pm 0.01& &  4.432 \pm 0.006& &  1.4030 \pm 0.0008& \\
& & \textsc{Ode} &  5.3287 \pm 0.0004& &  8.949 \pm 0.002& &  4.419 \pm 0.002& &  1.4018 \pm 0.0001& \\
& & \textsc{Cl} &  5.3281 \pm 0.0003& &  8.949 \pm 0.002& &  4.410 \pm 0.002& &  1.40155 \pm .00009& \\
\addlinespace
% \hat{\sigma}^-
$\hat{\sigma}^- \pm \delta \hat{\sigma}^- \,\text{[pb]}$& & \Vegas &  -6.446 \pm 0.005e-4& &  -1.981 \pm 0.004& &  -9.810 \pm 0.008& &  -5.894 \pm 0.003& \\
& & \textsc{Ode} &  -6.450 \pm 0.001e-4& &  -1.9844 \pm 0.0006& &  -9.802 \pm 0.003& &  -5.8932 \pm 0.0005& \\
& & \textsc{Cl} &  -6.4488 \pm 0.0003e-4& &  -1.9821 \pm 0.0007& &  -9.800 \pm 0.002& &  -5.8918 \pm 0.0003& \\
\addlinespace
% \hat{\Sigma}^{\pm}\pm
$\hat{\Sigma}^{\pm}\pm \delta \hat{\Sigma}^{\pm} \,\text{[pb]}$& & \Vegas &  5.328 \pm 0.002& &  6.97 \pm 0.01& &  -5.38 \pm 0.01& &  -4.491 \pm 0.003& \\
& & \textsc{Ode} &  5.3281 \pm 0.0004& &  6.965 \pm 0.003& &  -5.381 \pm 0.004& &  -4.4914 \pm 0.0006& \\
& & \textsc{Cl} &  5.3274 \pm 0.0003& &  6.967 \pm 0.003& &  -5.390 \pm 0.004& &  -4.4903 \pm 0.0004& \\
\addlinespace
% \epsilon^{+}_{\Phi} 
$\epsilon^{+}_{\Phi}$& & \Vegas & 0.99& & 0.73& & 0.64& & 0.81& \\
& & \textsc{Ode} & 1.00& & 0.99& & 0.99& & 1.00& \\
& & \textsc{Cl} & 1.00& & 0.99& & 0.99& & 1.00& \\
\addlinespace
% \epsilon^{-}_{\Phi} 
$\epsilon^{-}_{\Phi}$& & \Vegas & 0.83& & 0.38& & 0.85& & 0.95& \\
& & \textsc{Ode} & 1.00& & 0.99& & 0.99& & 1.00& \\
& & \textsc{Cl} & 1.00& & 0.99& & 0.99& & 1.00& \\
\addlinespace
% \epsilon^+
$\epsilon^+$ & $\epsilon^+_{\text{0.1\%}}$ & \Vegas & 0.13 & 0.43& 0.048 & 0.098& 0.020 & 0.048& 0.082 & 0.21\\
& & \textsc{Ode} & 0.33 & 0.70& 0.025 & 0.30& 0.0059 & 0.099& 0.11 & 0.56\\
& & \textsc{Cl} & 0.53 & 0.81& 0.028 & 0.24& 0.0082 & 0.046& 0.17 & 0.63\\
\addlinespace
% \epsilon^-
$\epsilon^-$ & $\epsilon^-_{\text{0.1\%}}$ & \Vegas & 0.016 & 0.066& 0.013 & 0.021& 0.049 & 0.17& 0.12 & 0.27\\
& & \textsc{Ode} & 0.055 & 0.36& 0.028 & 0.17& 0.020 & 0.16& 0.12 & 0.73\\
& & \textsc{Cl} & 0.11 & 0.79& 0.0074 & 0.060& 0.0090 & 0.19& 0.40 & 0.79\\

==> table-performance-NNLO-RR.tex <==
Contribution $\sigma^i$ & & & $\sigma^{\mathrm{RRF}} \cdot 10^{-2}$& & $\sigma^{\mathrm{RRSU}} \cdot 10^{-3}$& & $\sigma^{\mathrm{RRDU}} \cdot 10^{-3}$ & \\
$\delta_{\mathrm{opt}}$ [pb] & & &  0.008& &  0.004& &  0.01& \\
cost $C_i$ [a.u.]& & & 53& & 26& & 8 & \\
% \hat{\sigma}
$\hat{\sigma} \pm \delta \hat{\sigma}\,\text{[pb]}$& & \Vegas &  -0.30 \pm 0.02 & &  2.835 \pm 0.007& &  -2.46 \pm 0.02 & \\
& & \textsc{Ode} &  -0.33 \pm 0.01& &  2.823 \pm 0.005& &  -2.42 \pm 0.02 & \\
& & \textsc{Cl} &  -0.32 \pm 0.01& &  2.829 \pm 0.004& &  -2.41 \pm 0.01 & \\
\addlinespace
% \hat{\sigma}^+
$\hat{\sigma}^+ \pm \delta \hat{\sigma}^+\,\text{[pb]}$& & \Vegas &  3.82 \pm 0.01& &  3.718 \pm 0.006& &  5.639 \pm 0.007 & \\
& & \textsc{Ode} &  3.812 \pm 0.006& &  3.706 \pm 0.003& &  5.644 \pm 0.004 & \\
& & \textsc{Cl} &  3.814 \pm 0.005& &  3.704 \pm 0.003& &  5.643 \pm 0.004 & \\
\addlinespace
% \hat{\sigma}^-
$\hat{\sigma}^- \pm \delta \hat{\sigma}^-\,\text{[pb]}$& & \Vegas &  -4.14 \pm 0.01& &  -0.881 \pm 0.002& &  -8.078 \pm 0.009 & \\
& & \textsc{Ode} &  -4.142 \pm 0.006& &  -0.885 \pm 0.005& &  -8.071 \pm 0.007 & \\
& & \textsc{Cl} &  -4.134 \pm 0.006& &  -0.885 \pm 0.002& &  -8.076 \pm 0.005 & \\
\addlinespace
% \hat{\Sigma}^{\pm}
$\hat{\Sigma}^{\pm} \pm \delta \hat{\Sigma}^{\pm}\,\text{[pb]}$& & \Vegas &  -0.31 \pm 0.03& &  2.836 \pm 0.008& &  -2.44 \pm 0.02 & \\
& & \textsc{Ode} &  -0.33 \pm 0.01& &  2.821 \pm 0.007& &  -2.43 \pm 0.01 & \\
& & \textsc{Cl} &  -0.32 \pm 0.01& &  2.819 \pm 0.004& &  -2.433 \pm 0.009 & \\
\addlinespace
% \epsilon^{+}_{\Phi}
$\epsilon^{+}_{\Phi}$& & \Vegas & 0.54& & 0.73& & 0.80 & \\
& & \textsc{Ode} &  0.84& & 0.96& & 0.99 & \\
& & \textsc{Cl} &  0.86& & 0.95& & 0.98 & \\
\addlinespace
% \epsilon^{-}_{\Phi}
$\epsilon^{-}_{\Phi}$& & \Vegas & 0.51& & 0.40& & 0.80 & \\
& & \textsc{Ode} &  0.85& & 0.83& & 0.98 & \\
& & \textsc{Cl} &  0.85& & 0.84& & 0.99 & \\
\addlinespace
% \epsilon^+
$\epsilon^+$ & $\epsilon^+_{\text{0.1\%}}$ & \Vegas & 0.0040 & 0.0052& 0.0073 & 0.017& 0.0018 & 0.022\\
& & \textsc{Ode} &  0.0013 & 0.0027& 0.0028 & 0.022& 0.0030 & 0.023\\
& & \textsc{Cl} &  0.0022 & 0.0056& 0.0096 & 0.022& 0.0029 & 0.011\\
\addlinespace
% \epsilon^-
$\epsilon^-$ & $\epsilon^-_{\text{0.1\%}}$ & \Vegas & 0.0041 & 0.0053& 0.0035 & 0.010& 0.0037 & 0.019\\
& & \textsc{Ode} &  0.0019 & 0.0053& 0.00025 & 0.00025& 0.0018 & 0.0096\\
& & \textsc{Cl} &  0.0034 & 0.0060& 0.0012 & 0.0028& 0.0044 & 0.011\\

==> table-performance-NNLO-V.tex <==
Contribution $\sigma^i$ & & & $\sigma^{\mathrm{RVF}} \cdot 10^{-2}$& & $\sigma^{\mathrm{RVFR}} \cdot 10^{-2}$& &
$\sigma^{\mathrm{RVDU}} \cdot 10^{-3}$& & $\sigma^{\mathrm{VVF}} \cdot 1$& \\
$\delta_{\mathrm{opt}}$ [pb] & & &  0.008& &  0.002& &  0.005& &  0.01& \\
cost $C_i$ [a.u.]& & & 1542& & 3& & 3& & 13& \\
% \hat{\sigma}
$\hat{\sigma} \pm \delta \hat{\sigma}\,\text{[pb]}$& & \Vegas &  -6.81 \pm 0.02& &  0.286 \pm 0.002& &  0.267 \pm 0.005& &  14.77 \pm 0.01& \\
& & \textsc{Ode} &  -6.784 \pm 0.008& &  0.289 \pm 0.002& &  0.271 \pm 0.005& &  14.76 \pm 0.01& \\
& & \textsc{Cl} &  -6.778 \pm 0.008& &  0.285 \pm 0.002& &  0.276 \pm 0.005& &  14.77 \pm 0.01& \\
\addlinespace
% \hat{\sigma}^+
$\hat{\sigma}^+ \pm \delta \hat{\sigma}^+\,\text{[pb]}$& & \Vegas &  1.669 \pm 0.003& &  1.051 \pm 0.001& &  2.381 \pm 0.001& &  16.711 \pm 0.007& \\
& & \textsc{Ode} &  1.6764 \pm 0.0009& &  1.0495 \pm 0.0004& &  2.3806 \pm 0.0004& &  16.720 \pm 0.003& \\
& & \textsc{Cl} &  1.676 \pm 0.002& &  1.0500 \pm 0.0006& &  2.3799 \pm 0.0004& &  16.718 \pm 0.002& \\
\addlinespace
% \hat{\sigma}^-
$\hat{\sigma}^- \pm \delta \hat{\sigma}^-\,\text{[pb]}$& & \Vegas &  -8.454 \pm 0.007& &  -0.764 \pm 0.001& &  -2.111 \pm 0.001& &  -1.955 \pm 0.001& \\
& & \textsc{Ode} &  -8.458 \pm 0.002& &  -0.7627 \pm 0.0003& &  -2.1109 \pm 0.0005& &  -1.9554 \pm 0.0002& \\
& & \textsc{Cl} &  -8.456 \pm 0.003& &  -0.7626 \pm 0.0006& &  -2.1091 \pm 0.0004& &  -1.9548 \pm 0.0001& \\
\addlinespace
% \hat{\Sigma}^{\pm}
$\hat{\Sigma}^{\pm} \pm \delta \hat{\Sigma}^{\pm}\,\text{[pb]}$& & \Vegas &  -6.785 \pm 0.009& &  0.287 \pm 0.003& &  0.270 \pm 0.002& &  14.756 \pm 0.008& \\
& & \textsc{Ode} &  -6.781 \pm 0.003& &  0.2868 \pm 0.0006& &  0.2697 \pm 0.0009& &  14.765 \pm 0.003& \\
& & \textsc{Cl} &  -6.780 \pm 0.005& &  0.287 \pm 0.001& &  0.2708 \pm 0.0008& &  14.763 \pm 0.002& \\
\addlinespace
% \epsilon^{+}_{\Phi}
$\epsilon^{+}_{\Phi}$& & \Vegas & 0.55& & 0.59& & 0.95& & 0.96& \\
& & \textsc{Ode} &  0.99& & 0.99& & 1.00& & 1.00& \\
& & \textsc{Cl} &  0.99& & 0.98& & 1.00& & 1.00& \\
\addlinespace
% \epsilon^{-}_{\Phi}
$\epsilon^{-}_{\Phi}$& & \Vegas & 0.87& & 0.50& & 0.92& & 0.82& \\
& & \textsc{Ode} &  0.99& & 0.98& & 1.00& & 1.00& \\
& & \textsc{Cl} &  0.99& & 0.99& & 1.00& & 1.00& \\
\addlinespace
% \epsilon^+
$\epsilon^+$ & $\epsilon^+_{\text{0.1\%}}$ & \Vegas & 0.013 & 0.024& 0.025 & 0.060& 0.029 &
0.22& 0.015 & 0.10\\
& & \textsc{Ode} &  0.0029 & 0.067& 0.0081 & 0.099& 0.030 & 0.27& 0.0086 & 0.49\\
& & \textsc{Cl} &  0.00076 & 0.00076& 0.0024 & 0.035& 0.010 & 0.22&
0.020 & 0.31\\
\addlinespace
% \epsilon^-
$\epsilon^-$ & $\epsilon^-_{\text{0.1\%}}$ & \Vegas & 0.014 & 0.038& 0.021 & 0.050& 0.011 & 0.11& 0.024 & 0.17\\
& & \textsc{Ode} &  0.051 & 0.25& 0.017 & 0.095& 0.017 & 0.18& 0.17 & 0.49\\
& & \textsc{Cl} &  0.0054 & 0.13& 0.0017 & 0.018& 0.022 & 0.22& 0.10 & 0.68\\
